Universal and data-adaptive algorithms for model selection in linear contextual bandits

Model selection in contextual bandits is an important complementary problem to regret minimization with respect to a fixed model class. We consider the simplest non-trivial instance of model-selection: distinguishing a simple multi-armed bandit problem from a linear contextual bandit problem. Even in this instance, current state-of-the-art methods explore in a suboptimal manner and require strong "feature-diversity" conditions. In this paper, we introduce new algorithms that a) explore in a data-adaptive manner, and b) provide model selection guarantees of the form $\mathcal{O}(d^{\alpha} T^{1- \alpha})$ with no feature diversity conditions whatsoever, where $d$ denotes the dimension of the linear model and $T$ denotes the total number of rounds. The first algorithm enjoys a "best-of-both-worlds" property, recovering two prior results that hold under distinct distributional assumptions, simultaneously. The second removes distributional assumptions altogether, expanding the scope for tractable model selection. Our approach extends to model selection among nested linear contextual bandits under some additional assumptions.

==> abstract.tex <==
\begin{abstract}
This writeup provides an algorithm that achieves model selection in over linear contextual bandits with model orders $d_1 < \ldots < d_M$ with rates of the form $\mathcal{O}(d_{i^*}^{\alpha} T^{1 - \alpha})$, where $i^* \in [M]$ is the index of the true model and $\alpha \in (0,1)$ is a fixed parameter.
Unlike past work, the only assumption that we make is that the contexts are stochastic and $1$-sub-Gaussian.
Our estimator uses a combination of eigenvalue thresholding and an double debiasing estimator of what is currently the ``simpler" model.
Next, we present an adaptive algorithm for model selection that adapts the value of $\alpha$ according to the ``easiness" of the instance in a MAB-vs-contextual-bandit model selection problem.
The main ingredient in this algorithm is a data-adaptive exploration schedule.
\end{abstract}

==> ideasdataadaptive.tex <==
\section{Data-adaptive exploration in MAB-vs-contextual-bandit}

In this section, we present a data-adaptive model selection algorithm for \textit{multi-armed-bandits-vs-contextual bandits} (MAB v.s. CB).
Concretely, we consider a linear CB instance with hidden MAB structure as follows:
\begin{align*}
    g_{i,t} = \lin{\alpha_{i,t},\Tstar} + \mu_{i} + W_{i,t} ,
\end{align*}

where $W_{i,t}$ denotes iid sub-Gaussian noise (with parameter $\sigma^2$), $\{\mu_i\}_{i \in [K]}$ denote the biases, and $\alpha_{i,t}$ denotes the context process, which we will assume (only in this section) to be iid across $t \geq 1$ for every $i$.
We will denote the two model classes as follows:
\begin{itemize}
    \item Simple model (SM) denotes the case in which $\Tstar = 0$ and the problem is actually a MAB instance. 
    Let $i^*$ denote the optimal arm, i.e. $i^* \in {\arg \max} \mu_i$.
    If we knew this in advance, the optimal instance-dependent regret would be $\Oh\left(\sum_{i \neq i^*} \min\{\frac{\log T}{\Delta_i}, \Delta_i T\}\right)$, and the optimal minimax regret would be $\Oh(\sqrt{T})$.
    \item Complex model (CM) denotes the case in which $\Tstar \neq 0$ and the problem is a CB instance.
    Here, the optimal minimax regret will be $\Oh((\sqrt{d} + \sqrt{K})\sqrt{T})$. \ak{The $\sqrt{K}$ factor arises because we must also learn the $\mu_i$s.}
\end{itemize}
Our aim in this section is to construct algorithms that achieve the optimal rate under the strong assumptions considered in~\citet{chatterji2020osom}, but also achieve positive model selection rates under weaker conditions.
We will do this by designing a data-adaptive exploration schedule.
Before presenting the meta-method, we state our assumptions on contextual information and construct certain confidence sets which are standard in the literature.

\subsection{Assumptions on contexts}

First, we assume that the contexts are stochastic and iid across rounds as well as independent across rounds\footnote{As in~\citet{chatterji2020osom}, the iid assumption can be relaxed to a stochastic process with upper and lower bounds on the covariance matrix, but for now we restrict to the iid case for simplicity in exposition.}.
For convenience, we also assume that the contexts are centered and bounded, so
\begin{align*}
    \mathbb{E}\left[\alpha_{i,t}\right] &= \mathbf{0} \\
    \lv \alpha_{i,t} \rv_2^2 &\leq d .
\end{align*}

It is also convenient to assume that the context vectors are all sub-Gaussian with parameter at most $1$.
(This is $\tau$ in~\citet{foster2019model}.)
This assumption of sub-Gaussianity was made in both~\cite{chatterji2020osom,foster2019model}.
We denote the second-moment matrix of the context $\alpha_{i,t}$ by $\Sigma_i$.

In addition to the above mild assumptions, the following stronger eigenvalue assumptions were made in previous work.
\begin{enumerate}
    \item The strongest of the assumptions concerned the minimum eigenvalue of all contexts individually. 
    In other words, it stated that $\gamma_{min}(\Sigma_i) \geq \loweig > 0$ for a dimension-independent constant $\loweig$.
    Under this assumption, optimal model selection is known to be possible because (at a high level) external exploration is not needed~\cite{chatterji2020osom}.
    Henceforth, we call this condition the \textit{universal eigenvalue condition}.
    \item A relatively weaker assumption is on the minimum eigenvalue of the \textit{action-averaged} covariance matrix, i.e. $\gamma_{min}(\overline{\Sigma}) \geq \loweig > 0$ where $\overline{\Sigma} := \frac{1}{K} \sum_{i=1}^K \Sigma_i$.
    Under this assumption,~\citet{foster2019model} show suboptimal but non-trivial model selection results.
    Henceforth, we call this condition the \textit{action-averaged eigenvalue condition}.
\end{enumerate}

An related assumption to the action-averaged eigenvalue assumption is: there exists $i_0 \in [K]$ (unknown to the algorithm designer) such that $\gamma_{min}(\Sigma_{i_0}) \geq \loweig$.
We call this the \textit{existence of an eigenvalue assumption}. \ak{Is it obvious that this assumption helps more than some $\textrm{poly}(K)$ factor? If I told you $i_0$, you may still have to play it frequently (and hence incur regret) to get a well-conditioned second moment matrix.} 
\vm{Yes, you are right. I think I am going to omit this bullet point entirely as I am now unsure it is a value-add.}

\subsection{Construction of Confidence Sets}
In our algorithm, which is presented subsequently at the \emph{end of round} $t$, we build an upper confidence estimate for each arm. Let $T_i(t): = \sum_{s=1}^t \mathbb{I}\left[A_s = i\right]$ be the number of times arm $i$ was pulled and $\averagerew := \sum_{s=1}^t g_{i,s}\mathbb{I}\left[A_s = i\right]/T_i(t)$ be the average reward of that arm at the end of round $t$. For each arm we define the upper confidence estimate for any $\delta' > 0$:
\begin{align}
    &\label{def:ucbarms}
    \muit{i}{t} : = \averagerew + \sigma\left[\frac{1+T_{i}(t)}{T_{i}^2(t)}\left(1+ 2\log\left(\frac{K(1+T_i(t))^{\frac{1}{2}}}{\delta'}\right)\right)\right]^{\frac{1}{2}}.
\end{align}
  Lemma~6 in \citep{abbasi2011improved} (restated below as Lemma~\ref{lem:csimplebound} here) uses a refined self-normalized martingale concentration inequality to bound $\lvert \mu_i - \averagerew \rvert$ across all arms and all rounds. 

\begin{lemma}\label{lem:csimplebound} Under the simple model, with probability at least $1-\delta'$ we have, for all $i \in \{1,\ldots,K\}$ and for all $t\ge 0$,
\begin{align*}
     \lvert \mu_i - \averagerew \rvert\le \sigma\left[\frac{1+T_{i}(t)}{T_{i}^2(t)}\left(1+ 2\log\left(\frac{K(1+T_i(t))^{\frac{1}{2}}}{\delta'}\right)\right)\right]^{\frac{1}{2}}.
\end{align*}
\end{lemma}

We will also construct estimates $\That$ for $\Tstar$ for use if we know that the model is complex.
For any round $t>K$, let $\That$ be the $\ell^2$-regularized least-squares estimate of $\Tstar$ defined below.
\begin{align}
\label{def:ohat}
\That = \left(\Aboldt^{\top}\Aboldt +  I\right)^{-1} \Aboldt^{\top} \Gboldt,
\end{align}
where $\Aboldt$ is the matrix whose rows are the context vectors selected from round $K+1$ up until round $t$: $\alpha_{A_{K+1},K+1}^{\top},\ldots,\alpha_{A_t,t}^{\top}$ and $\Gboldt = [g_{A_{K+1},K+1}- \tilde{\mu}_{A_{K+1},K},\ldots,g_{A_t,t}- \muit{A_t}{t-1}]^{\top}$. Here we are regressing on the rewards seen to estimate $\theta^*$, while using the bias estimates $\muit{i}{t-1}$ obtained by our upper confidence estimates defined in Eq.~\eqref{def:ucbarms}.
\begin{restatable}{lemma}{thetaset}\label{prop:thetaconfidence} Let $\That$ be defined as in Eq.~\eqref{def:ohat}. Then, with probability at least $1-3\delta'$ we have that for all $t>K$, $\theta^*$ lies in the set
\begin{align}
\mathcal{C}_{t}^c &: = \left\{\theta\in \mathbb{R}^d: \lv \theta - \That\rv_{2} \le \kenvt \right\},
 \label{def:ccomplex}
\end{align}
where $\kenvt = \widetilde{\mathcal{O}}\left(\sigma \sqrt{\frac{d}{t}}\right)$.
\end{restatable}
% We prove this lemma in Appendix~\ref{app:omittedproofs}.


Finally, we define the estimate of the signal $S := \lv \theta^* \rv_2^2$ as below.
This estimator is inspired by the work of~\citet{verzelen2018adaptive} and was refined by~\citet{foster2019model}.
We denote this estimator by $\widehat{S}_t$.
This estimator will be used in the interrim model selection step.

\subsection{The meta-method} 

\begin{algorithm}[t]
\caption{Model Selection Through One-Shot Sequential Testing \label{algorithm:OFULER}}


\For{$t=1,\ldots,K$}{
Play arm $t$ and receive reward $g_{t,t}$, \qquad \emph{\text{(Play each arm at least once.)}}
}
\For{$t=K+1,\ldots,n$}{
    ${\texttt{Current Model}} \leftarrow \text{`Simple'}$
     
    \textit{Simple Model Estimate: } \begin{align}\label{eq:simpleestimate}
        i_t = \text{ arm pulled by a gap-optimal regret bound (e.g. UCB~\cite{auer2002finite}) }
    \end{align} \\
    \textit{Complex Model Estimate:
    }
    \begin{align}\label{eq:complexestimate}
        j_t = \text{ arm pulled by the OFUL/LinUCB~\cite{chu2011contextual,abbasi2011improved} algorithm }
    \end{align}\\
    % where $\mathcal{C}_{t-1}^c$ defined in Eq.~\eqref{def:ccomplex}.

    \If{${\emph{\texttt{Current Model}} = \text{`Simple'}}$ and $t> K+1$} {Check the condition: 
    \begin{align} \label{test:complextest} 
    \Sgaphat(\W(t)) \le \alpha_{\delta'}(|\W(t)|,T)^2, 
    \end{align}
    where $\wenvone$ will be defined subsequently, and $\Sgaphat(\W(t))$ is a constructed estimator of $||\Tstar||^2$ (which is an upper bound on the gap between the two models) defined subsequently. Here, $\W(t)$ is the set of designated ``exploration" rounds which will be defined shortly.
    
    If violated then set ${\texttt{Current Model}} \leftarrow \text{`Complex'}$.
    }
    
    If ${\texttt{Current Model}}=\text{`Simple'}$: Play arm $A_t$, as defined subsequently, and receive reward $g_{A_t,t}$. Let $\W(t)$ denote the set of designated ``exploration" rounds as will be defined shortly.\\
    
    Else if ${\texttt{Current Model}}=\text{`Complex'}$: Play arm $j_t$ and receive $g_{j_t,t}.$
    
    Update $\left\{\tilde{\mu}_{i,t}\right\}_{i=1}^K$ and $\ccomplex$.
        
    }    
\end{algorithm}


Algorithm~\ref{algorithm:OFULER} describes the ``meta-method" for model selection.
The two building blocks of the meta-method, that are not yet described, are the choice of action $A_t$ when the current model is detected as simple, and the choice of estimator $\widehat{G}_{\W(t),max}$ for the maximal obtainable reward using the best-in-class linear model, i.e. $G_{\W(t),max}$.
The former choice determines an \textit{exploration schedule}, whose choice impacts the regret incurred by both the simple and complex models. 
On the other hand, the estimation error of the latter choice determines the fidelity of the model selection bound in the case of the complex model.
In other words, the parameter $\alpha_{\delta'}(|\W(t)|,T)$ constitutes an upper bound on the estimation error $G_{\W(t),\max} - \widehat{G}_{\W(t),\max}$ that holds with probability at least $1 - \delta'$.
% The algorithms in~\citet{chatterji2020osom,foster2019model} differ, roughly speaking, in their choices of exploration schedule and estimator.
% We detail these choices below.

% \begin{definition}\label{def:osom}
% The algorithm $\algname$ does no forced exploration, i.e. $A_t = i_t$ when the current state of the model is simple, and plugs in the optimistic estimate for $\Tstar$, based on what the complex model would have recommended, into an estimator as below:
% \begin{align}\label{eq:osomestimate}
%     \widehat{G}_{t-1,max} := \sum_{s=K}^{t-1} \tilde{\mu}_{j_s,s-1}+\langle \alpha_{j_s,s},\tilde{\theta}_s \rangle .
% \end{align}
% \end{definition}

% It is worth briefly justifying the choices made by $\algname$.
% The choice of $A_t = i_t$ is what ensures optimal rates for the simple model, and can be leveraged because of the universal eigenvalue condition, allowing exploration to occur automatically while the simpler model is being exploited. 
% Moreover, we can show that the estimator as defined in Equation~\eqref{eq:osomestimate} is a good one.
% This follows by a useful lower bound on $\widehat{G}_{t-1,max}$: using the definition of the optimistic estimate we get
% \begin{align*}
%     \sum_{s=K}^{t-1} \tilde{\mu}_{j_s,s-1}+\langle \alpha_{j_s,s},\tilde{\theta}_s \rangle &\geq \sum_{s=K}^{t-1} \tilde{\mu}_{\kappa_s,s-1}+\langle \alpha_{\kappa_s,s},\tilde{\theta}_s \rangle \\
%     \implies G_{t-1,max} - \widehat{G}_{t-1,max} &\leq \sum_{s=K}^{t-1} \mu_{\kappa_s} - \tilde{\mu}_{\kappa_s,s-1} + \langle \alpha_{\kappa_s,s},(\Tstar - \tilde{\theta}_s) \rangle .
% \end{align*}

% (At a high level), the dominating term is the second one, and it can be shown to scale (with probability at least $1 - \delta'$) as $\wenv := \mathcal{O}_{\delta'}(\sqrt{dt})$ in both cases - whether the model is simple or complex.
% However, this guarantee critically relies on the \textit{universal eigenvalue condition} $\gamma_{\min}(\Sigma_i) \geq \loweig$ for all $i \in [K]$.
% Putting these observations together (details in proofs in~\citet{chatterji2020osom}), it is easy to show that the instance-optimal guarantee is obtained under the simple model, and the minimax optimal guarantee is possible in the complex model.
% (See the main theorem there for formal statements.)
% {\color{blue} The hidden constant in $\wenvone$ has a factor of $\frac{\higheig}{\loweig}$; therefore, knowledge of these parameters is unfortunately needed.}

% \begin{definition}\label{def:modcb}
% The algorithm $\mathsf{ModCB}$ {\color{blue}(modified to this setting by me)} uses forced exploration in the following way:
% \begin{align*}
%     A_t = \begin{cases}
%     i_t \text{ w.p. } (1 - \mu_t) \\
%     \text{Unif}[K] \text{ w.p. } \mu_t ,
%     \end{cases}
% \end{align*}

% where $\mu_t = t^{-1/3}$, and constructs the estimate for $\widehat{G}_{t-1,max}$ as {\color{blue}(as interpreted by me for this setting)}
% \begin{align*}
%     \widehat{G}_{t-1,max} := \sum_{s=K}^{t-1} \tilde{\mu}_{i_s,s-1} + 2 (t-1) \sqrt{\higheig \cdot \widehat{S}_{t-1} } \geq \sum_{s=K}^{t-1} \tilde{\mu}_{\kappa_s,s-1} + 2 (t-1) \sqrt{\higheig \cdot \widehat{S}_{t-1} }
% \end{align*}
% where $\widehat{S}_{t-1}$ is the estimate of the norm $S := ||\Tstar||_2^2$ as motivated by~\citet{verzelen2018adaptive} and refined in~\citet{foster2019model}.
% {\color{blue} Vidya: note that the algorithm designer will not have access to $\kappa_s$ as it is a function of $\Tstar$.}
% \end{definition}

% Observe that the expected number of exploration rounds will scale as $n^{2/3}$, and this leads to a regret of $\mathcal{O}(n^{2/3})$ for the simple model.
% For the complex model, it is straightforward to upper bound
% \begin{align*}
%     G_{t-1,max} &\leq \sum_{s=K}^{t-1} \mu_{\kappa_s} + 2(t-1) \sqrt{\higheig \cdot S }
% \end{align*}

% with high probability.
% (This follows from the sub-Gaussian assumption that we made on all contexts for all actions and an anytime Hoeffding bound.)

% Therefore, the estimation error $G_{t-1,max} - \widetilde{G}_{t-1,max}$ is dominated by the quantity $\sqrt{\widehat{S}_{t-1}} - \sqrt{S}$, which can be shown to scale as $\mathcal{O}_{\delta'}\left(\frac{d^{1/4}}{\text{poly}(\loweig) \cdot \sqrt{T_e(t)}}\right)$ with probability at least $1 - \delta'$, where $T_e(t)$ denotes the number of forced-exploration rounds, i.e. rounds where we chose $A_t \sim \text{Unif}[K]$.
% {\color{blue} Vidya: I have not checked the dependencies on $\higheig, \loweig$ carefully yet, so there could be mistakes here.}
% By our choice of exploration schedule, we get $T_e(t) \sim t^{2/3}$, and so the overall estimation error can be easily verified to scale as
% \begin{align*}
%     G_{t-1,max} - \widehat{G}_{t-1,max} \leq \sum_{s=K}^{t-1} \mu_{\kappa_s} - \tilde{\mu}_{\kappa_s,s-1} + \mathcal{O}_{\delta'}(d^{1/4} t^{2/3}) ,
% \end{align*}

% and this gives a regret bound of $\mathcal{O}(d^{1/4} n^{2/3})$ for complex model instances that are treated as simple.
% On the other hand, for complex instances detected as such we would get regret $\mathcal{O}(\sqrt{d n})$.

% {\color{blue} It is easy to combine the ``greedy" procedure for action selection in $\algname$ with the improved estimator used by $\mathsf{ModCB}$ if we knew that we had the nice universal eigenvalue condition.
% Then, $T_e(t) = t$, and the dominating term in the estimation error rate would become $\mathcal{O}_{\delta'}(d^{1/4} t^{1/2})$, and we get the following trifecta of rates:
% \begin{enumerate}
%     \item Regret under SM continues to be instance-optimal w.h.p.
%     \item Regret under CM which is detected as simple will be $\mathcal{O}_{\delta'}(d^{1/4} n^{1/2})$.
%     \item Regret under CM detected as complex will (trivially) be $\mathcal{O}_{\delta'}(\sqrt{dn})$.
% \end{enumerate}

% Thus, the worst-case rates do not change, but we get an improved rate for relatively benign instances that are technically in the complex model, i.e. $\Tstar \neq 0$.
% }

% We will next use this observation to design a ``first-cut" adaptive exploration algorithm.
% By default, we will use the improved estimator $\widehat{G}_{t-1,max}$ that uses the estimation of signal, i.e. $\widehat{S}_{t-1}$.

\subsection{Data-adaptive exploration}

Our goal in this section to design an exploration schedule with the following (crude) adaptive guarantee:
\begin{enumerate}
    \item Under the \textit{universal eigenvalue condition}, we get the trifecta of optimal rates.
    % {\color{blue} (Might also consider a weaker condition of $\gamma_{\min}(\Sigma_{i^*}) \geq \loweig$, where $i^*$ maximizes \\ $\{\mu_i, i \in [K]\}$, in the future. This would slightly change the exploration protocol in the beginning, so I omit it for now for simplicity.)}
    \item Under the \textit{action-averaged eigenvalue condition} or \textit{existence of an eigenvalue assumption}, we get the trifecta of suboptimal rates $n^{2/3}$ for SM and $\max\{d^{1/4} n^{2/3}, \sqrt{dn}\}$ for CM. 
    % {\color{blue} Note the possibility of these rates for the existence of an eigenvalue assumption as well.}
\end{enumerate}

We define our adaptive exploration schedule below.
\begin{definition}\label{def:dataadaptive}
Our data-adaptive exploration schedule under the simple model maintains an ``exploration" set that we will define shortly, denoted by $S(1) \subseteq S(2) \ldots \subseteq S(\tauswitch)$, where $\tauswitch$ denotes the switching time to the complex model (if it exists).
It takes as input the parameter $\loweig > 0$ and uses the covariate matrix $M_{t-1} := \sum_{s \in S(t-1)} \alpha_{A_s,s} \alpha_{A_s,s}^\top$ designed at round $t$.
Further, we define the new covariate matrix $M_t(i) := M_{t-1} + \alpha_{i,t} \alpha_{i,t}^\top$.
We define two such schedules.
The first one is designed to work with the universal eigenvalue condition and the action-averaged eigenvalue condition.
We define a random variable $Z_t \sim \text{Bernoulli}(1 - \mu_t)$, and the random variable
\begin{align*}
    Y_t = \mathbb{I}\left[\frac{1}{t} \cdot \gamma_{\min}(M_t(i_t)) \geq \frac{\loweig}{2}\right].
\end{align*}
Based on these, we define the following exploration schedule:
\begin{align}\label{eq:explorationschedule1}
    A_t = \begin{cases}
    i_t \text{ if } Y_t = 1 \text{ or } Z_t = 1.\\
    \sim \text{Unif}[K] \text{ otherwise. } 
    \end{cases}
\end{align}
We fix $\mu_t = t^{-1/3}$ as in $\mathsf{ModCB}$.
Next, we explicitly define the exploration set that we will use for the model selection estimator as:
\begin{align*}
    \W(t) := \{1 \leq s \leq t: Y_s = 1 \oplus Z_s = 0 \}.
\end{align*}
% \vm{Logical check: we do not want to include the alternative scenarios: a) $Y_t = 0$ and $Z_s = 1$ implies that the minimum eigenvalue condition was not met AND we did not do forced exploration. Therefore, these samples will not give us the estimation of squared loss gap guarantee that we require. b) $Y_t = 1$ and $Z_s = 0$ are samples for which there may be bias in estimation from estimating the mean parameters $\{\mu_i\}_{i \in [K]}$, so we do not want to include them.}
We will only use the set of rounds $\W(t)$ to construct the estimator $\Sgaphat(\W(t))$ at every round $t > 1$.
% \vm{Currently written informally}
We also define the set of ``forced exploration" rounds as 
\begin{align*}
    \T(t) := \{1 \leq s \leq t: Y_s = 0 \text{ and } Z_s = 0.\}
\end{align*}
Note that, by definition, $\T(t)$ denotes the subset of exploration rounds $\W(t)$ for which the minimum-eigenvalue condition (indicated by $Y_s = 1$) is \textit{not} met.
Finally, we will only deploy the data-adaptive exploration schedule \textit{and} model selection test after $t \geq \tau_{\min}(\delta,T) := \left(\frac{16}{\loweig^2} + \frac{8}{3 \loweig} \right) \log \left(\frac{2dT}{\delta}\right)$; for all $t < \tau_{\min}(\delta,T)$ we will just use the SM by default.
\vm{Revisit and see whether we actually require this}
\end{definition}

% \ak{I think there might be a problem here. Now, before we switch, the way we choose the action $A_t$ looks at the current features $\alpha_{t,i}$. Specifically this is true in the first case for in~\eqref{eq:explorationschedule1}. The problem is that our estimate of $\mu_i$ crucially uses that the features are centered, so that even if we are in the complex model, their contribution can be viewed as noise. But if our action $i_t$ depends on the feature $\alpha_t$, then we are introducing some bias into these estimates. Maybe this is handled somehow? (I think this is ok in the universal eigenvalue case since we always play $A_t = i_t$. But not sure about the other case.)}

% \vm{(July 7) fix: use the fact that the number of such ``bad case" rounds is atmost $T^{2/3}$ w.h.p. and ignore mean reward samples from this case. Therefore number of samples used for estimation still scales linearly in $T$. Show that all regret bounds unaffected as well as statistical test. (July 12): modified the definitions above to reflect this fix. We will characterize $|\W(t)|$ and $|\T(t)|$ for all cases below. What we have below is still a proof sketch, but should be fairly straightforward to flesh out at this point.}

For convenience, we index the elements of $\W(t)$ in ascending order by $s_1,\ldots,s_{|\W(t)|}$.
We define our estimator of $\Sgaphat(\W(t))$ below:
\begin{align}
    \Sgaphat(\W(t)) := \frac{1}{\binom{|\W(t)|}{2}} \sum_{j' < j} \Big{\langle} \Sigmahat_t^{-1/2} x_{s_{j'}} y_{s_{j'}}, \Sigmahat_t^{-1/2} x_{s_j} y_{s_j} \Big{\rangle} ,
\end{align}
where $x_s := \alpha_{s,A_s}$, $y_s = g_{s,A_s} - \widetilde{\mu}_{s,A_s}$ and $\Sigmahat_t$ denotes the sample covariance matrix collected at time $t$ of the \textit{average} covariance matrix, i.e.
\begin{align}
    \Sigmahat_t := \frac{1}{(t-1)K} \sum_{s=1}^{t-1} \sum_{i=1}^K \alpha_{s,i} \alpha_{s,i}^\top .
\end{align}
\vm{Analyzing this estimator will require more sophisticated martingale arguments than in~\citet{foster2019model}, as we are using heterogeneous and adaptively collected samples for the $x,y$'s. I am writing this shortly as a separate lemma.}
% \vm{Not yet defined formally, but will be a simple modification of the ``square-loss-gap" estimator that is also used in~\citet{foster2019model}}

We state and prove the following result on model selection regret, for a fixed $\gamma > 0$.
\begin{theorem}\label{thm:dataadaptive}
For any $\gamma > 0$ have the following results for model selection between MAB and CB:
\begin{enumerate}
    \item If the universal eigenvalue condition holds for parameter $\loweig' \geq \loweig$, we get
    \begin{subequations}\label{eq:universalmodelselection}
    \begin{align}
        R_T^S &= \Oh\left(\sum_{i \neq i^*} \frac{1}{\Delta_i}\log\left(\frac{2KT}{\Delta_i \delta}\right)\right) \text{ and } \\
        R_T^C &= \Oh\left(\left(\sqrt{\frac{d}{\loweig'}} + \sqrt{K}\right)\sqrt{T}\right)
    \end{align}
    \end{subequations}
    w.p. at least $1 - \delta$.
    \item If the action-averaged eigenvalue condition holds for parameter $\gamma' \geq \gamma$, we get
    \begin{subequations}\label{eq:actionaveragedmodelselection}
    \begin{align}
        R_T^S &= \Oh(\sqrt{KT} + T^{2/3}) \text{ and } \\
        R_T^C &= \Oh\left(\frac{1}{(\loweig')^2} K^{1/4} d^{1/4} T^{2/3}\right)
    \end{align}
    \end{subequations}
\end{enumerate}
\end{theorem}
Observe that Equation~\eqref{eq:universalmodelselection} is identical to the OSOM rate, and Equation~\eqref{eq:actionaveragedmodelselection} is identical to the ModCB rate.
Our data-adaptive exploration subroutine results in a \textit{single} algorithm that achieves both rates under the requisite conditions.
(In general, OSOM will not work under the action-average eigenvalue condition, and the rate of ModCB does not improve under the universal eigenvalue condition.)

We provide a proof (sketch) of Theorem~\ref{thm:dataadaptive} below.
\begin{proof}
Our proof sketch will constitute of a deterministic proof working on various events used in~\citet{chatterji2020osom} and~\citet{foster2019model} as well as additional events that we will show are high-probability.
\paragraph{Meta-analysis:}

We begin the analysis by providing a common lemma for both cases that will characterize a high-probability regret bound as a functional of two random quantities $|\W(t)|$, the total number of exploration rounds, and $|\T(t)|$, the total number of forced-exploration rounds.
First, we state our guarantee on estimation error.
\begin{lemma}\label{lem:esterrordataadaptive}
For every $t \geq 1$, we have
\begin{align}\label{eq:esterrordataadaptive}
    |\Sgaphat(\W(t)) - \Sgaptilde| &\leq \frac{1}{2} \Sgaptilde + \mathcal{O}\left(\frac{\sigma^2}{\gamma^2} \cdot \frac{d^{1/2} \log^2(2d/\delta)}{|\W(t)|} + \frac{1}{\gamma^4} \cdot \frac{d + \log(2/\delta)}{t}\right)
\end{align}
with probability at least $1 - \delta$, where we define
\begin{align*}
    \Sgaptilde := ||\Sigmabar^{-1/2} \Sigmabar_t \Tstar||_2^2.
\end{align*}
We denote $\alpha_{\delta}(s,t) := \Oh\left(\frac{\sigma^2}{\gamma^2} \cdot \frac{d^{1/2} \log^2(2d/\delta)}{|\W(t)|} + \frac{1}{\gamma^4} \cdot \frac{d + \log(2/\delta)}{t}\right)$ as shorthand.
% \vm{All factors above to be slightly changed/modified after proof is completely written. In particular dependences on $\gamma$ may change.}
\end{lemma}

\begin{proof}
\vm{Ignores error terms in estimating $\mu_i$'s for now; this should not be difficult because our definition of $\W(t)$ ensures that such samples are unbiased.}
Similar to the proof of Theorem~\ref{thm:truncatedestimator}, the analysis proceeds in two parts (the third part of bounding the truncation-related error is not needed for the moment as we are not using truncation anywhere):
% \begin{enumerate}
%     \item Upper-bounding $|\Sgaphat(\W(t)) - \E{\Sgaphat(\W(t))}|$, where expectation is taken only over the noisy samples $\{x_{j_s},y_{j_s}\}_{j = 1}^{|\W(t)|}$. This will give us the first error term in the analysis. \vm{Clarifying question (also relevant for~\cite{foster2019model} because there as well we used $\sum_{s=1}^t$ for the estimate of $\Sigmahat$): is it important that the samples used for estimating $\Sigmahat_t$ are on disjoint rounds from $\W(t)$?}
%     \item Upper-bounding $|\E{\Sgaphat(\W(t))} - \Sgap|$.
%     This will give us the second error term in the analysis as all of the error in estimating $\Sigmahat_t$ is from $t$ unlabeled samples.
% \end{enumerate}

\textit{1. Upper-bounding $\left|\Sgaphat(\W(t)) - \Sgapbar(\W(t))\right|$,} where we define
\begin{align*}
    \Sgapbar(\W(t)) &:= ||\Sigmahat_t^{-1/2} \Sigmabar_t \Tstar||_2^2, \text{ where } \\
    \Sigmabar_t &:= \frac{1}{|\W(t)|} \E{\sum_{j=1}^{|\W(t)|} x_{s_j} x_{s_j}^\top}.
\end{align*}
Note that $\Sigmabar_t$ is a random quantity, because $\W(t)$ is a random subset of $[t]$. Also note that by our sub-Gaussian assumption, we have $\Sigmabar_t \preceq I$ a.s.
\vm{More details needed here to avoid the $\sqrt{\log K}$ upper bound (although that's not super consequential either way): we considered the samples $\W(t)$ for which the choice of $i_t$ either did not depend on the context realizations, OR we did forced exploration. So the $x_{s_j}$'s are always centered and then we just use $\Sigma_i \preceq I$ for all $i \in [K]$.}
% We note that $\E{\Sgaphat} = ||\Sigmahat^{1/2}(\Tstar_1 - \Omegahat \E{xy})||_2^2$.
For a given index $1 \leq j \leq |\W(t)|$, we consider the random vector
\begin{align*}
    \Sigmahat_t^{-1/2} x_{s_j} y_{s_j} - \Sigmahat_t^{-1/2} \E{x_{s_j} y_{s_j} |\H_{s_j - 1} },
\end{align*}

and show that it is conditionally sub-exponential with parameter $\mathcal{O}(2/ \gamma)$.
Consequently, using a martingale version of the sub-exponential tail bound, we get 
\begin{align*}
    \left|\Sgaphat(\W(t)) - \Sgapbar(\W(t))\right| &= \mathcal{O}\left(\frac{1}{\gamma} \cdot \frac{d^{1/2} \log^2(2d/\delta)}{|\W(t)|} + \frac{1}{\sqrt{\gamma}} \cdot \frac{||\Sigmahat_t^{-1/2} \Tstar||_{2} \log(2/\delta)}{\sqrt{|\W(t)|}}\right) .
\end{align*}
with probability at least $1 - \delta$ for all $t \geq 1$.
\vm{TODO: fill in specific martingale concentration lemma for concreteness}

Now, we note that $\sqrt{\gamma} \cdot ||\Sigmahat_t^{-1/2} \Tstar||_{2} \leq \sqrt{\Sgapbar(\W(t))}$.
Therefore, we apply the AM-GM inequality to deduce that
\begin{align}\label{eq:prooffirstpartada}
    \left|\Sgaphat(\W(t)) - \Sgapbar(\W(t))\right| &\leq \frac{1}{8} \Sgapbar(\W(t)) +  \mathcal{O}\left(\frac{1}{\gamma^2} \cdot \frac{d^{1/2} \log^2(2d/\delta)}{|\W(t)|} \right).
\end{align}
% \vm{Note the slightly worse scaling in minimum-eigenvalue $\gamma$ that ensues from the ``transfer" in covariate distributions between averaging over actions (used to estimate $\Sigmahat_t$ with unlabeled samples) and exploration set (which is collected adaptively). Maybe possible to improve this but I'm not 100\% sure yet.}

\textit{2. Upper-bounding $\left|\Sgapbar(\W(t)) - \Sgaptilde\right|$.}
We note that $\Sgaptilde = ||\Sigmabar^{-1/2} \Sigmabar_t \Tstar||_2^2$, and $\Sgapbar(\W(t)) := ||\Sigmahat_t^{-1/2} \Sigmabar_t \Tstar||_2^2$, where recall that $\Sigmabar$ denotes the action-averaged covariance matrix.
Further, recall that $\Sigmahat_t$ is the sample covariance matrix constructed from $t$ \textit{unlabeled} samples.
Thus, applying Lemma~\ref{lem:opnormcontrol}, following an identical sequence of steps to~\citet{foster2019model}, and using that $\Sigmabar_t \preceq I$ and $||\Tstar||_2 \leq 1$, we get
\begin{align}\label{eq:proofsecondpartada}
    \left|\Sgapbar(\W(t)) - \Sgaptilde\right| \leq \frac{1}{8} \Sgaptilde + \Oh\left(\frac{1}{\gamma^4} \cdot \frac{d + \log(2/\delta)}{t}\right).
\end{align}
Now, putting Equations~\eqref{eq:prooffirstpartada} and~\eqref{eq:proofsecondpartada} together, we get
\begin{align*}
    |\Sgaphat(\W(t)) - \Sgaptilde| \leq \frac{1}{2} \Sgaptilde + \mathcal{O}\left(\frac{1}{\gamma^2} \cdot \frac{d^{1/2} \log^2(2d/\delta)}{|\W(t)|} + \frac{1}{\gamma^4} \cdot \frac{d + \log(2/\delta)}{t} \right).
\end{align*}
This completes the proof.
\vm{Note that $\Sgaptilde$ will have an extra $\frac{1}{\gamma}$ scaling in it owing to the mismatch between $\Sigmabar_t$, which incorporates adaptive sampling, and $\Sigmabar$, which only uses action-averaging. This leads to an extra $\frac{1}{\gamma}$ scaling which we state formally in the next lemma.}
\end{proof}


Next, we prove the following meta-lemma that characterizes the simple and complex model regret purely in terms of $\W(T)$ and $\T(T)$ with high probability.
\begin{lemma}\label{lem:metaanalysis}
For any $\gamma > 0$ and $\delta > 0$, the following result holds with probability at least $1 - \delta$ for model selection between MAB and CB:
\begin{align*}
    R_T^S &= \Oh\left(\sum_{i \neq i^*} \frac{1}{\Delta_i} \log \left(\frac{2KT}{\Delta_i \delta}\right) + |\T(T)| \right) \text{ and } \\
    R_T^C &= \Oh\left(|\T(T)| + \sqrt{dT}\left(1 + \frac{1}{\gamma^3}\right) + \frac{d^{1/4}}{\gamma^2} \cdot \frac{T}{\sqrt{|\W(T)|}}\right)
\end{align*}
\end{lemma}

\begin{proof}
For this proof, we define $\alpha_{\delta'}(\W(t),t,T)$ as a high-probability upper bound on the estimation error $\Sgaptilde - \Sgaphat(\W(t))$, where $\Sgaptilde$ was defined in Lemma~\ref{lem:esterrordataadaptive}.
% We will specify the value of $\alpha_{\delta'}(\W(t),t,T)$ shortly, and use it as a black-box to complete the proof.
More concretely, we will work on the event
\begin{align*}
    \Ecal_0 := \{\left|\Sgaptilde - \Sgaphat(\W(t))\right| \leq \frac{1}{2} \Sgaptilde + \alpha_{\delta'}(\W(t),T)^2 \text{ for all } t = 1,\ldots,T\},
\end{align*}
where $\alpha_{\delta'}(\W(t),t,T)$ is as defined in Equation~\eqref{eq:esterrordataadaptive}.
\vm{we added the extra index $T$ because actually, we will use an anytime concentration bound for the martingale steps there which will add a logarithmic dependence on $T$ even for $t < T$}
Lemma~\ref{lem:esterrordataadaptive} showed that this happens with probability at least $1 - \delta$.
% \vm{Some paraphrasing of that statement will be needed: because $|\W(t)|$ is itself random, we will take an anytime martingale concentration bound in that lemma which will provide a $\log(T)$ dependence.}
% \vm{This is just a rephrasing of the usual square-loss-gap bound, e.g.~\citet[Theorem 2]{foster2019model}.}
Further, we denote $g_{\max} = \E{\max_{i \in [K]} \alpha_i^\top \Tstar + \mu_i}$.
We now have two cases to analyze:
\begin{enumerate}
    \item The case where the true model is SM.
    In this case, note that $\Sgaptilde = 0$ by definition and the event $\Ecal_0$ directly gives us, for all $t \geq 1$,
    \begin{align*}
    \Sgaphat(\W(t)) \leq 0 + 0 + \alpha_{\delta'}(\W(t),T)^2
    \end{align*}
    w.h.p. and so the condition for elimination is never met.
    Since under this event, we stay in the complex model, we get pseudo-regret
    \begin{align*}
        R_T^S &\leq \sum_{t \notin \T(T)} (\mu^* - \mu_{A_t}) + |\T(T)| \\
        &= \sum_{t \notin \T(T)} (\mu^* - \mu_{i_t}) + |\T(T)| \\
        &= \Oh\left(\sum_{i \neq i^*} \frac{1}{\Delta_i} \log \left(\frac{2KT}{\Delta_i \delta}\right) + |\T(T)|\right).
    \end{align*}
    Above, the first step uses that rewards are bounded. The second step uses that by the definition of $\T(T)$ and the fact that we never switch, we will have $A_t = i_t$ for all $t \notin \T(T)$. The third step uses the fact that SM updates are only made using the rounds that are not ``forced-exploration", i.e. not in $\T(T)$. \vm{I don't think I made this explicit in the algorithm definition 
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    
    but it's probably important for clean analysis}
    This completes the proof of the lemma for the case of SM.
    \item The case where the true model is CM.
    Let $\tauswitch$ denote the round at which the algorithm switches to CM, if any (otherwise, we define $\tauswitch := T$).
    It suffices to bound the regret until time $\tauswitch$ (when we will be playing the SM).
    First, we note that because we are in $t \leq \tauswitch$, we must have $\Sgaphat(\W(t)) \leq \alpha_{\delta'}(\W(t),T)^2$.
    Therefore, we get
    \begin{align*}
        \Sgaptilde \leq 2 \Sgaphat(\W(t)) + \alpha_{\delta'}(\W(t),T)^2 \leq 3 \alpha_{\delta'}(\W(t),T)^2.
    \end{align*}
    Furthermore, we note that $\Sgaptilde \geq ||\Tstar||_2^2 \cdot \gamma^2$ (because we have $\Sigmabar_t \succeq \gamma I$ and $\Sigmabar^{-1/2} \succeq I$), which gives us 
    \begin{align}\label{eq:snrbound}
        ||\Tstar||_2^2 \leq \frac{3}{\gamma^2} \cdot  \alpha_{\delta'}(\W(t),T)^2.
    \end{align}
    Next, we get
    \begin{align*}
        R_T^C &= \sum_{t=1}^{\tauswitch} (\alpha_{t,\kappa_t}^\top \Tstar + \mu_{\kappa_t} - \alpha_{t,A_t}^\top \Tstar - \mu_{A_t}) \\
        &\leq \sum_{t \notin \T(\tauswitch)} (\alpha_{t,\kappa_t}^\top \Tstar + \mu_{\kappa_t} - \alpha_{t,i_t}^\top \Tstar - \mu_{i_t}) + |\T(T)| \\
        &\leq T \cdot ||\Tstar||_2 + \sum_{t \notin \T(\tauswitch)} \mu^* - \mu_{i_t} + |\T(T)|\\
        &\leq \frac{T}{\gamma} \cdot \alpha_{\delta'}(\W(\tauswitch),T) + \sum_{i \neq i^*} \frac{1}{\Delta_i} \log \left(\frac{2KT}{\Delta_i \delta}\right) + |\T(T)| \\
        &= \Oh\left(|\T(T)| + \sqrt{dT}\cdot \frac{1}{\gamma^3} + \frac{d^{1/4}}{\gamma^2} \cdot \frac{T}{\sqrt{|\W(T)|}}\right).
    \end{align*}
    \vm{I have not yet included the bias-terms in the regret analysis for SM owing to adaptive exploration. It should be workable but will be a bit complicated. It may make life a bit simpler to use Exp3 as the SM algorithm instead, but then we'd sacrifice the instance-dependent guarantees.}
    This completes the proof for the case of CM as well.
    The first step is the definition of regret. The second step uses the definition of $\T(T)$ and the fact that we have not switched yet. The third step uses a sub-Gaussian tail bound (and might incur $\log K$ factors). The fourth step uses Equation~\eqref{eq:snrbound}. The fifth step substitutes the definition of $\alpha_{\delta}(\cdot,\cdot)$ from Equation~\eqref{eq:esterrordataadaptive}.
    \vm{Note the extra $\gamma$ factor that arises as a consequence of transfer between the adaptively collected exploration samples and the estimation quantity of interest.}
\end{enumerate}

\end{proof}

% \vm{Proof sketch of Lemma~\ref{lem:metaanalysis} below}
% In all cases, the proof will proceed by analyzing two situations:
% \begin{enumerate}
%     \item True model = SM: here, we will show that w.h.p., we will never switch over to the complex model in either of the cases.
%     \vm{Note that this does not depend in any way on the evolution of $|S(t)|$ with $t$.}
%     Here, the regret will be equal to SM regret + $\Oh(|T(T)|)$ = $\Oh\left(\frac{\log T}{\Delta} + |T(T)|\right)$, and thus precise upper bounds on $|T(T)|$ will suffice to complete the analysis for this case.
%     \item True model = CM. Let the round at which the switch is made be $\widehat{T}$ (or $T$ if this switch is never made).
%     In a manner of analysis that is identical to~\citet{foster2019model}, we will get the meta-result
%     \begin{align*}
%         R_T^C = \Oh\left(|T(T)| + \sqrt{dT} + \widehat{T} \sqrt{\alpha_{\widehat{T}-1}}\right)
%     \end{align*}
%     \vm{Fast estimation used here; essence of result will not change because we always ensure the min-eigenvalue condition + unbiasedness of estimators. TODO: fill in details about this}
    
%     where (as a consequence of the data-adaptive schedule), we will define
%     \begin{align*}
%         \alpha_{t} := C_1 \cdot \frac{1}{\gamma^4} \cdot \frac{d^{1/2}}{|S(t)|} + \frac{1}{\gamma^8} \cdot \frac{d}{t} .
%     \end{align*}
%     \vm{log factors and dependences on $K$ omitted above for brevity}
%     As a consequence, and noting that $\widehat{T} \leq T$, we get
%     \begin{align}\label{eq:metaregretcomplex}
%         R_T^C = \Oh\left(|T(T)| + \sqrt{dT} + \frac{d^{1/4}}{\gamma^2} \cdot \frac{T}{\sqrt{|S(T)|}} + \frac{1}{\gamma^2} \cdot \sqrt{dT} \right)
%     \end{align}
%     Therefore, precise characterizations of the number of ``forced exploration" rounds $T(T)$ and overall exploration rounds $S(T)$ will suffice to complete the analysis for this case.
% \end{enumerate}

% We will start with the case for which the minimum-eigenvalue condition holds, i.e. $\gamma_{\min}(\Sigma_i) \geq \gamma > 0$ for all $i \in [K]$.

\paragraph{Case 1: Universal eigenvalue condition holds}

As in~\citet{chatterji2020osom}, we need to show that $Y_t = 1$ for all $t \geq 1$ w.h.p. in order to get the desired regret bound.
Note that this directly ensures that $A_t = i_t$ for all $t \geq 1$.
This requires showing two high-probability events.
The first defined below:
\begin{align}
    \Ecal_1 := \left\{Y_t = 1 \text{ for all }  t \in \{\tau_{\min}(\delta,T),\ldots,T\}\right\}.
\end{align}
We now show that the event $\Sgap_1$ occurs with probability at least $1 - \delta$.
Since $i_t$ is a deterministic functional of the history $\H_{t-1}$, we can apply~\cite[Lemma 7]{chatterji2020osom} (which is an application of the matrix Freedman inequality) to get
\begin{align*}
    \gamma_{\min}(M_t(i_t)) \geq 1 + \frac{\loweig t}{2} \text{ for all } t \geq \tau_{\min}(\delta,T) 
\end{align*}
with probability at least $1 - \delta$.
This clearly ensures that $\frac{1}{t} \cdot \gamma_{\min}(M_t(i_t)) \geq \frac{\gamma}{2} \text{ for all }  t \in \{\tau_{\min}(\delta,T),\ldots,T\}$, which is the required condition.

Connecting this to the meta-analysis above, event $\Ecal_1$ ensures that $|\T(T)| = 0$ by the definition of $\T(t)$.
This completes the proof for the case where the true model is SM.

For the case of CM, we also need to \textit{lower bound} $|\W(T)|$.
Note that $|\W(T)|$ is lower bounded by the number of rounds $1 \leq t \leq T$ for which $Y_t = 1$ and $Z_t = 1$.
Since $Z_t \sim \text{Bernoulli}(1 - \mu_t)$ and independent of $\{Y_t\}$, on the event $\Ecal_1$ we have
\begin{align*}
    |\W(T)| \geq \sum_{t=1}^T Z_t \geq T(1 - 2T^{-1/3}) \geq T/2
\end{align*}
where the last inequality follows for large enough $T$, and the second-to-last inequality is a consequence of the Hoeffding bound.
Plugging this into Lemma~\ref{lem:metaanalysis} completes the proof of the theorem.

% \paragraph{Case 2: Universal eigenvalue condition holds, CM:}

% Next, we consider the case where $\Tstar \neq 0$, i.e. we are in the complex model case, and the universal eigenvalue condition continues to hold.
% Note that $\Ecal_1$ continues to hold for this case with probability at least $1 - \delta$, and so we will always select $A_t = i_t$ as long the model is detected as ``simple", implying that $S(t) = t$ for all $1 \leq t \leq \tauswitch$.
% Moreover, we consider the event $\Ecal'_2$ that the regret under the CM is $\Oh((\sqrt{d} + \sqrt{K})\sqrt{T})$ as long as $A_t = i_t$ and the condition in Equation~\eqref{test:complextest} is never violated.
% By an analysis identical to that of~\citet{chatterji2020osom}, this event occurs with probability at least $1 - \delta$ as well.
% Finally, we consider the event $\Ecal'_0$ that the CM regret is upper-bounded by $\Oh((\sqrt{d} + \sqrt{K})\sqrt{T})$, and note by standard analyses of LinUCB/OFUL~\cite{chu2011contextual,abbasi2011improved} that this is a high-probability event as well.
% Thus, taking a union bound over the events $\Ecal_0,\Ecal_1,\Ecal_2$ completes the proof for this case.

% Next, we consider the case where the action-averaged eigenvalue condition holds, but not necessarily the universal eigenvalue condition.
% For this proof, we will use the testing framework and analysis of~\citet{foster2019model}.

% Let $\tauswitch$ denote the (random) round, if it exists, at which the procedure switches from detecting the model from simple to complex.
% % Further, we denote by
% % \begin{align*}
% %     \mathcal{S}(\tauswitch) := \{1 \leq t \leq \tauswitch: A_t = i_t \text{ or } Z_t = 1 \}
% % \end{align*}
% % the set of ``guaranteed-exploration" rounds.
% Overloading notation, we also denote $M_{S(t)} := I + \sum_{s \in S(t)} \alpha_{s,A_s} \alpha_{s,A_s}^\top$ to be the regression matrix used to estimate the square loss gap.
% This is simply the regression matrix that is built up from designated ``exploration" rounds.
% We state two facts that will be essential for the proof for both the SM and CM case.
% \begin{enumerate}
%     \item Our designated exploration-rounds satisfy the desired minimum-eigenvalue condition, i.e. $\frac{1}{|S(t)|} \cdot \gamma_{\min}(M_{S(t)}) \geq \frac{\gamma}{2}$ for all $t \geq \tau_{\min}(\delta,T)$ with probability at least $1 - \delta$.
%     This is because the two conditions for membership in $S(t)$ are $A_s = i_s$ or $Z_s = 1$.
%     In the former case, this condition is \textit{deterministically} met; in the latter case, the action-averaged eigenvalue condition guarantees that this will hold (recall from Definition~\ref{def:dataadaptive} that $Z_s = 1$ and $A_s \neq i_s$ would ensure that $A_s \sim \text{Unif}[K]$).
%     \item The number of exploration rounds scales as $t^{2/3}$, i.e. we have $\frac{t^{2/3}}{2} \leq |S(t)| \leq  2 t^{2/3}$ with high probability as a consequence of the Hoeffding bound over the $Z_s$'s as in prior analysis~\cite{foster2018contextual,lee2021online}, and noting that $Z_s = 1$ is a sufficient condition for membership in $S(t)$.
% \end{enumerate}

% The proof follows as a rather elementary application of these two facts coupled with prior analysis, as sketched below.

\paragraph{Case 2: Action-averaged eigenvalue condition holds}
In the case where the action-averaged eigenvalue condition holds, it suffices to provide an upper bound on $|\T(T)|$ and a lower bound on $|\W(T)|$.
We will not define any extra statistical events for this case.
First, we note that 
\begin{align*}
    |\T(T)| \leq |\{1 \leq t \leq T: Z_s = 0\}| \leq 2 \sum_{t=1}^T \mu_t \leq 4 T^{2/3}
\end{align*}
where the second-to-last inequality again follows with high probability by the Hoeffding bound.
This gives us SM minimax regret that scales as $\Oh(T^{2/3})$.
(We completely sacrifice on the instance-dependent guarantees in this case.)

On the other hand, we use the fact that $\{Z_t\}_{t \geq 1}$ is a randomized sequence completely independent of everything else to get
\begin{align*}
|\W(T)| &= |\{1 \leq t \leq T: Y_t = 1 \text{ and } Z_t = 1\}| + |\{1 \leq t \leq T: Y_t = 0 \text{ and } Z_t = 0 \}| \\
&\geq 0.5 |\{1 \leq t \leq T: Y_t = 1\}| + |\{1 \leq t \leq T: Y_t = 0\}|^{2/3} \\
&\geq 0.5 |\{1 \leq t \leq T: Y_t = 1\}|^{2/3} + |\{1 \leq t \leq T: Y_t = 0\}|^{2/3} \\
&\geq 0.5 (T/2)^{2/3} = \omega(T^{2/3}).
\end{align*}
Above, the second inequality used an anytime Hoeffding bound over the independent random variables $\{Z_t\}_{t = 1}^T$.

Plugging these bounds into Lemma~\ref{lem:metaanalysis} gives us
\begin{align*}
    R_T^C = \Oh\left(T^{2/3} + \sqrt{dT} + \frac{1}{\gamma^2} \cdot \sqrt{dT} + \frac{d^{1/4} T^{2/3}}{\gamma^2}\right),
\end{align*}
which completes the proof for this case.
\end{proof}



==> ideasnoeigenvalue.tex <==
\section{Eigenvalue thresholding for ``universal" model selection}

In this section, we formalize the estimator that uses eigenvalue thresholding, and its estimation error guarantee on the square loss gap.
We will consider $n$ labeled samples, and $m$ unlabeled samples, with $m \gg n$.
\vm{Note: in the contextual bandit application we will consider $m \sim T$ and $n \sim T^{1 - \kappa}$, where $\kappa$ is an exploration parameter.}

\subsection{Setup and notation}
We borrow the notation from~\citet{foster2019model}, and define only additional notation here.
We will use the new estimator $\Sigmahat$ from \textit{unlabeled} samples $\{\tildex_s\}_{s=1}^m$.
These estimators are defined below.

\begin{definition}\label{def:thresholdingoperator}
For any positive semidefinite matrix $A$ that has diagonalization $M := U_M \Lambda_M U_M^\top$, and any $\gamma > 0$, we define the thresholding operator 
\begin{align*}
    \Tgamma{M} &:= U_M \Tgamma{\Lambda_M} U_M^\top \text{ where } \\
    \Tgamma{\Lambda} &= \text{diag}(\lambda_1(\gamma),\ldots,\lambda_d(\gamma)) \text{ and } \\
    \lambda(\gamma) &:= \max\{\lambda, \gamma\} .
\end{align*}
\end{definition}

We use Definition~\ref{def:thresholdingoperator} to specify our (biased) estimators of the covariance matrices $\Sigma, \Omega := \Sigma^{-1}$.
In particular, we let $\Sigmahat^{(m)}$ denote the sample covariance matrix of $\Sigma$.
Then, our estimators are given by
\begin{subequations}
\begin{align}
    \Sigmahat &:= \Tgamma{\Sigmahat^{(m)}} \label{eq:sigmaestimate} \\
    \Omegahat &:= \Sigmahat^{-1} \label{eq:sigmainverseestimate} .
\end{align}
\end{subequations}
Note that $\Sigmahat$ is always invertible.

\vm{Estimators of $\Sigma_1$ and its inverse are removed, as we are essentially not using the fast estimator for simple-model terms. Also, come back to this after writing full proof: we may only require the truncation operator for $\Omegahat$.}

Finally, we will write $\Tstar := \begin{bmatrix} \Tstar_1 & \Tstar_{-1} \end{bmatrix}$, where $\Tstar_1 \in \R^{d_1}$ and $\Tstar_{-1} \in \R^{(d - d_1)}$.
We will overload notation and write $\Tstar_1 := \begin{bmatrix} \Tstar_1 & 0 \end{bmatrix} \in \R^d$ as the $d$-dimensional version of $\Tstar_1$ padded with $(d - d_1)$ zeros.
We define
\begin{align}\label{eq:squaregaptodebiased}
    \Sgap' := \E{(x^\top \Tstar_1 - x^\top \Tstar)^2} ,
\end{align}

and note two important properties of $\Sgap'$:
\begin{enumerate}
    \item $\Sgap' \geq \Sgap$ by the definition of the MMSE estimate under simple model of order $d_1$.
    \item When the model order is simple, we have $\Sgap' = \Sgap = 0$.
\end{enumerate}

Using these observations, we will seek an estimator of $\Sgap'$, and use it for model selection rather than $\Sgap$.

\subsection{Estimation guarantee with side information}
Our initial algorithm uses as side-information the parameter $\Tstar_1 \in \R^{d_1}$.
Later, we will estimate this parameter from $m \gg n$ independent labeled samples using a double-debiasing estimator.

\begin{algorithm}[H]
	\caption{ EstimateResidualWithSideInfo} \label{alg:estimateresidualsideinfo}
		\STATE \textbf{Input}: Examples $\{(x_s,y_s)\}_{s=1}^n$, second moment matrix estimate $\Sigmahat \in \R^{d \times d}$ and first $d_1$ signal components, $\Tstar_1$.
		\STATE Return estimator
		\begin{align*}
	    \Sgaphat := \frac{1}{\binom{n}{2}} \sum_{s < t} \Big{\langle} \Sigmahat^{1/2} (\Tstar_1 - \Omegahat x_s y_s), \Sigmahat^{1/2} (\Tstar_1 - \Omegahat x_t y_t) \Big{\rangle}
		\end{align*}
	\end{algorithm}

The following theorem (intended to replace Theorem 2 in~\citet{foster2019model}) characterizes the estimation error $|\Sgaphat - \Sgap|$ will depend on the choice of $\gamma$.

\begin{theorem}\label{thm:truncatedestimator}
Provided that $m \geq C(d + \log(2/\delta))/\gamma$, the estimator provided in Algorithm~\ref{alg:estimateresidualsideinfo} guarantees that
\begin{align*}
    |\Sgaphat - \Sgap'| &\leq \frac{1}{2} \Sgap' + \mathcal{O}\left(\frac{\sigma^2}{\gamma^2} \cdot \frac{d^{1/2} \log^2(2d/\delta)}{n} + \frac{1}{\gamma^4} \cdot ||\E{xy}||_2^2 \cdot \frac{d + \log(2/\delta)}{m} +\gamma \right) 
\end{align*}
with probability at least $1 - \delta$.
\end{theorem}

Before proving Theorem~\ref{thm:truncatedestimator}, let us explore its ramifications for an overall model selection rate for the case of bandit v.s. contextual bandit (i.e. only $2$ model classes and $d_1 = 0$).
{\color{blue} VM -- This is currently a proof sketch, not a fully written proof}
Note that substituting the value of $\epsilon$ gives us the overall rate
\begin{align*}
    |\Sgaphat - \Sgap| \leq \frac{1}{2} \Sgap + \mathcal{O}\left(\frac{1}{\gamma^2} \cdot \frac{d^{1/2} \log^2(2d/\delta)}{n} + \frac{1}{\gamma^4} \cdot \frac{d \log (2/\delta)}{m} \cdot ||\E{xy}||_2^2 + \gamma \right) .
\end{align*}

Substituting this into final expressions for regret (Appendix C.2.4 in~\citet{foster2019model}, paragraph marked as ``Final result") will give us:
\begin{align*}
    R_T &\leq \widetilde{\mathcal{O}}\left(\sqrt{\log(2/\delta)} K^{\kappa} T^{1 - \kappa} + \frac{1}{\gamma^2} \cdot K^{\frac{1}{2}(1 - \kappa)} \cdot T^{\frac{1}{2}(1 + \kappa)} \cdot d^{1/4} \log (2/\delta) + \frac{1}{\gamma^4} \cdot \sqrt{KT d \log^2(2/\delta)} + \gamma T \right) .
\end{align*}

Note that the extra $\gamma T$ term comes from the estimation misspecification error term that we are now incurring.
We now need to select $\gamma,\kappa$ to minimize the above expression.
\textit{One way} of setting the terms is given by equating the second and fourth terms, which gives
\begin{align*}
    \gamma^3 = \frac{d^{1/4}}{T^{\frac{1}{2}(1 -\kappa)}} .
\end{align*}

Substituting this into the above gives (ignoring dependences on $K$ for now)
\begin{align*}
    R_T \leq \widetilde{\mathcal{O}}\left(T^{1-\kappa} + d^{\frac{1}{12}} \cdot T^{\frac{5 + \kappa}{6}} + d^{\frac{1}{6}} \cdot T^{\frac{7 - 4\kappa}{6}} \right) .
\end{align*}

Then, substituting $\kappa = 1/2$ gives us
\begin{align*}
    RT_ \leq \widetilde{\mathcal{O}}\left(T^{1/2} + d^{1/12} \cdot T^{11/12} + d^{1/6} \cdot T^{5/6}\right) ,
\end{align*}

which is of the form we want! (i.e. $d^{\alpha} \cdot T^{1 - \alpha}$ for some $\alpha \in (0,1)$).

{\color{blue} VM -- just verified that if we instead equated the third and fourth terms, we'd get an overall rate of 
\begin{align*}
    T^{4/5} + d^{1/20} \cdot T^{4/5} + d^{1/10} \cdot T^{9/10} ,
\end{align*}

which also satisfies the relationship we want.          
}

Now that we understand the implications of Theorem~\ref{thm:truncatedestimator}, let us prove it.

\begin{proof}
Before beginning the proof, we define a term called the \textit{truncated square-loss gap} as below:
\begin{align}\label{eq:truncatedsquareloss}
   \Sgaptilde := (\Tstar_1 - \Tgamma{\Sigma}^{-1} \Sigma \Tstar)^\top \Tgamma{\Sigma} (\Tstar_1 - \Tgamma{\Sigma}^{-1} \Sigma \Tstar) .
\end{align}
% \ak{Above is $\widetilde{\Sgap}$?}
% \vm{Come back to this after finishing writing full proof: we may want to use the original estimator $\Sigmahat := \Sigmahat^{(m)}$ as a truncation step seems unnecessary for the covariance matrix estimation (may only be needed for the inverse).}

The proof is carried out in three distinct steps:
\begin{enumerate}
    \item Upper-bounding $\left|\Sgaphat - \E{\Sgaphat}\right|$, the ``variance" estimation error arising from $n$ samples.
    \item Upper-bounding $\left|\E{\Sgaphat} - \Sgaptilde\right|$, the bias-term with respect to the truncated squared loss gap.
    \item Upper-bounding $\left|\Sgaptilde - \Sgap\right|$, the bias arising from truncation.
\end{enumerate}

\textit{1. Upper-bounding $\left|\Sgaphat - \E{\Sgaphat}\right|$.}
We note that $\E{\Sgaphat} = ||\Sigmahat^{1/2}(\Tstar_1 - \Omegahat \E{xy})||_2^2$.
We consider the random vector
\begin{align*}
    \Sigmahat^{1/2}(\Tstar_1 - \Omegahat xy ) - \Sigmahat^{1/2} (\Tstar_1 - \Omegahat \E{xy}) ,
\end{align*}

and show that it is sub-exponential with parameter $\mathcal{O}(2/ \gamma)$.
This follows because $||\Sigmahat^{1/2} \Tstar_1 - \Sigmahat^{1/2} \Omegahat||_{\mathsf{op}} \leq 1 + ||\Omegahat^{1/2}||_{\mathsf{op}} \leq 1 +  \frac{1}{\sqrt{\gamma}} \leq \frac{2}{\sqrt{\gamma}}$, where the second-last inequality follows by the definition of the truncation operator.
\vm{Note: the $\sqrt{\gamma}$ scaling critically relies on $\Omegahat = \Sigmahat^{-1}$. Let's see if that helps us later in the eventual bound.}

Thus, using the sub-exponential tail bound just as in~\cite[Lemma 17]{foster2019model}, we get 
\begin{align*}
    \left|\Sgaphat - \E{\Sgaphat}\right| &= \mathcal{O}\left(\frac{1}{\gamma} \cdot \frac{d^{1/2} \log^2(2d/\delta)}{n} + \frac{1}{\sqrt{\gamma}} \cdot \frac{||\Sigmahat^{1/2} (\Tstar_1 - \Omegahat \E{xy})||_{2} \log(2/\delta)}{\sqrt{n}}\right) .
\end{align*}

Now, we note that $||\Sigmahat^{1/2} (\Tstar_1 - \Omegahat \E{xy})||_{2} = \sqrt{\E{\Sgaphat}}$.
Therefore, we apply the AM-GM inequality to deduce that
\begin{align}\label{eq:prooffirstpart}
    \left|\Sgaphat - \E{\Sgaphat}\right| &\leq \frac{1}{8} \E{\Sgaphat} +  \mathcal{O}\left(\frac{\sigma^2}{\gamma} \cdot \frac{d^{1/2} \log^2(2d/\delta)}{n} \right)
\end{align}

\textit{2. Upper-bounding $\left|\E{\Sgaphat} - \Sgaptilde\right|$.}

We denote $\mu := \E{xy}$ as shorthand.
Further, we denote $\Omega_{(1)}$ to be the $d \times d$ matrix whose first $d_1$ rows are the same as $\Omega$, and next $(d - d_1)$ rows are set to $0$.
\vm{One little snag here: assumes that $\Sigma$ is invertible, which is much weaker than an eigenvalue assumption but still an assumption.}
Then, by definition we get $\Tstar_1 = \Omega_{(1)} \mu$.
Thus, we can use the notation from~\citet{foster2019model} and set 
\begin{align*}
    \Rhat &:= \Omega_{(1)} - \Omegahat \\
    \widetilde{R} &:= \Omega_{(1)} - \Tgamma{\Sigma}^{-1} .
\end{align*}

It is then easy to verify that $\E{\Sgaphat} = \langle \Rhat \Sigmahat \Rhat \mu, \mu \rangle$ and $\Sgaptilde = \langle \widetilde{R} \Tgamma{\Sigma} \widetilde{R} \mu, \mu \rangle$.
Following an idential sequence of steps to~\citet{foster2019model}, we get
\begin{align*}
    \left|\E{\Sgaphat} - \Sgaptilde\right| \leq \frac{1}{8} \Sgaptilde + \mathcal{O}\left(||\Tgamma{\Sigma}^{-1/2} \Sigmahat (\widetilde{R} - \Rhat) \mu ||_2^2 + ||\Tgamma{\Sigma}^{-1/2} (\Sigmahat - \Tgamma{\Sigma}) \Rhat \mu||_2^2 + ||\Sigmahat^{1/2}(\widetilde{R} - \Rhat) \mu||_2^2 \right)
\end{align*}

Furthermore, note that $\Rhat - \widetilde{R} = \Tgamma{\Sigma}^{-1} - \Omegahat$, so we do not need to worry about the $\Omega_{(1)}$ terms.
We now state and prove the following lemma, which will help us characterize the sum above.

\begin{lemma}\label{lem:opnormcontrol}
We have
\begin{align}\label{eq:opnormcontrol}
    ||\Tgamma{\Sigma}^{-1/2} \Sigmahat \Tgamma{\Sigma}^{-1/2} - I||_{\mathsf{op}} &= \mathcal{O}(\epsilon) \text{ where } \\
    \epsilon := \frac{1}{\gamma} \cdot \sqrt{\frac{d + \log(2/\delta)}{m}} \nonumber
\end{align}

with probability at least $1 - \delta$.
From the above, we get the following inequalities:
\begin{subequations}\label{eq:opnormequations}
\begin{align}
    ||\Tgamma{\Sigma}^{-1/2} \Sigmahat||_{\mathsf{op}} &\leq \mathcal{O}(1) \label{eq:opnormequationsa} \\
    ||\Rhat \mu||_{2} &\leq \mathcal{O}(1/\gamma) \label{eq:opnormequationsb} \\
    ||\widetilde{R} - \Rhat||_{\mathsf{op}} &\leq \mathcal{O}(\epsilon/\gamma) \label{eq:opnormequationsc}
\end{align}
\end{subequations}
\end{lemma}

Before proving Lemma~\ref{lem:opnormcontrol}, we use it to complete the proof of Theorem~\ref{thm:truncatedestimator}.
Using Equation~\eqref{eq:opnormequations}, we get
\begin{align*}
    ||\Tgamma{\Sigma}^{-1/2} \Sigmahat (\widetilde{R} - \Rhat) \mu||_{\mathsf{op}}^2 &\leq ||\Tgamma{\Sigma}^{-1/2} \Sigmahat||_{\mathsf{op}}^2 ||\mu||_2^2 \cdot ||\widetilde{R} - \Rhat||_{\mathsf{op}}^2 \leq \mathcal{O}\left(\frac{||\mu||_2^2 \cdot \epsilon^2}{\gamma^2}\right) \\
    ||\Tgamma{\Sigma}^{-1/2} (\Sigmahat - \Tgamma{\Sigma}) \Rhat \mu||_2^2 &\leq ||\Tgamma{\Sigma}||_{\mathsf{op}} ||\Rhat \mu||_2^2 \cdot ||\Tgamma{\Sigma}^{-1/2} \Sigmahat \Tgamma{\Sigma}^{-1/2} - I||_{\mathsf{op}}^2 \leq \mathcal{O}\left(\frac{||\mu||_2^2 \cdot \epsilon^2}{\gamma^2}\right) \\
    ||\Sigmahat^{1/2}(\widetilde{R} - \Rhat) \mu||_2^2 &\leq ||\Sigmahat||_{\mathsf{op}} ||\mu||_2^2 \cdot ||\widetilde{R} - \Rhat||_{\mathsf{op}}^2 \leq ||\Sigmahat||_{\mathsf{op}} ||\mu||_2^2 \cdot ||\widetilde{R} - \Rhat||_{\mathsf{op}}^2 \leq \mathcal{O}\left(\frac{||\mu||_2^2 \cdot \epsilon^2}{\gamma^2}\right)
\end{align*}

This directly gives us
\begin{align}\label{eq:proofsecondpart}
    \left|\E{\Sgaphat} - \Sgaptilde\right| \leq \frac{1}{8} \Sgaptilde + \mathcal{O}\left(\frac{||\mu||_2^2 \cdot \epsilon^2}{\gamma^2}\right) .
\end{align}


\textit{3. Upper-bounding $\left|\Sgaptilde - \Sgap'\right|$.}
Observe that 
\begin{align*}
    \Sgaptilde &= \Tstar_1^\top \Tgamma{\Sigma} \Tstar_1 + \Tstar^\top \Sigma \Tgamma{\Sigma}^{-1} \Sigma \Tstar - 2\Tstar^\top \Sigma \Tstar_1 \\
    \Sgap' &= \Tstar_1^\top \Sigma \Tstar_1 + \Tstar^\top \Sigma \Tstar - 2\Tstar^\top \Sigma \Tstar_1 .
\end{align*}

This directly implies that
\begin{align*}
    |\Sgaptilde - \Sgap'| &= |\Tstar^\top (\Sigma \Tgamma{\Sigma}^{-1} \Sigma - \Sigma) \Tstar + \Tstar_1^\top(\Tgamma{\Sigma} - \Sigma) \Tstar_1 | \\
    &\leq |\Tstar^\top (\Sigma \Tgamma{\Sigma}^{-1} \Sigma - \Sigma) \Tstar| +  |\Tstar_1^\top(\Tgamma{\Sigma} - \Sigma) \Tstar_1| \\
    &\leq ||(\Sigma \Tgamma{\Sigma}^{-1} \Sigma - \Sigma)||_{\mathsf{op}} + 2 ||\Tgamma{\Sigma} - \Sigma||_{\mathsf{op}} ,
\end{align*}

where the second inequality follows because we have assumed bounded signal, i.e. $||\Tstar_1||_2 \leq ||\Tstar||_2 \leq 1$.
It remains to control the operator norm terms above.
It is easy to see that $||\Tgamma{\Sigma} - \Sigma||_{\mathsf{op}} \leq \gamma$.
For the other term, we denote $\Sigma := U \Lambda U^\top$, and note that $\Tgamma{\Sigma}^{-1} := U \Tgamma{\Lambda}^{-1} U^\top$.
Thus, we get
\begin{align*}
    ||(\Sigma \Tgamma{\Sigma}^{-1} \Sigma - \Sigma)||_{\mathsf{op}} &= ||(\Lambda \Tgamma{\Lambda}^{-1} \Lambda - \Lambda)||_{\mathsf{op}} \leq \gamma .
\end{align*}

Putting these together gives us
\begin{align}\label{eq:proofthirdpart}
    \left|\Sgaptilde - \Sgap'\right| \leq 2 \gamma .
\end{align}

Thus, putting together Equations~\eqref{eq:prooffirstpart},~\eqref{eq:proofsecondpart} and~\eqref{eq:proofthirdpart} completes the proof.
It only remains to prove Lemma~\ref{lem:opnormcontrol}, which we now do.
\begin{proof}
First, we note that Equation~\eqref{eq:opnormcontrol} directly implies Equations~\eqref{eq:opnormequationsa} and~\eqref{eq:opnormequationsb}.
To see this, we note the following in order:
\begin{enumerate}
    \item We have $||\Tgamma{\Sigma}^{-1/2} \Sigmahat||_{\mathsf{op}} \leq ||\Tgamma{\Sigma}^{-1/2} \Sigmahat \Tgamma{\Sigma}^{-1/2}||_{\mathsf{op}} ||\Tgamma{\Sigma}||_{\mathsf{op}} \leq (1 + \epsilon) = \mathcal{O}(1)$. This shows that Equation~\eqref{eq:opnormequationsa} holds.
    \item We have $||\Rhat||_{\mathsf{op}} = ||\Sigmahat^{-1}||_{\mathsf{op}} = \mathcal{O}(1/\gamma)$. This shows that Equation~\eqref{eq:opnormequationsb} holds.
    % \item $||\widetilde{R} - \Rhat||_{\mathsf{op}} = ||\Sigmahat^{-1} - \Tgamma{\Sigma}^{-1}||_{\mathsf{op}} \leq ||\Tgamma{\Sigma}^{-1}||_{\mathsf{op}} \cdot ||\Tgamma{\Sigma}^{-1/2} \Sigmahat \Tgamma{\Sigma}^{-1/2} - I||_{\mathsf{op}} \leq \epsilon/\gamma$. This shows that Equation~\eqref{eq:opnormequationsc} holds.
\end{enumerate}

We will next show Equation~\eqref{eq:opnormcontrol} and~\eqref{eq:opnormequationsc}, which will turn out to use similar arguments.
First, recall that $\Sigmahat := \Tgamma{\Sigmaha^{(m)}}$, and so we really want to upper bound the quantity $||\Tgamma{\Sigmahat^{(m)}} - \Tgamma{\Sigma}||_{\mathsf{op}}$.
It is well known (see, e.g.~\cite{boyd2004convex}) that for any positive semidefinite matrix $A$, the operator $\Tgamma{A} - \gamma I $ is a proximal operator with respect to the convex nuclear norm functional.
% {\color{blue} TODO: make citation a bit more formal in writing, maybe cite one of the SVT papers?}
The non-expansiveness of proximal operators then gives us
\begin{align*}
    &||\Tgamma{\Sigmahat^{(m)}}- \Tgamma{\Sigma}||_{\mathsf{op}} \\
    &= ||\Tgamma{\Sigmahat^{(m)}} - \gamma I - ( \Tgamma{\Sigma} - \gamma I)||_{\mathsf{op}} \\
    &\leq ||\Sigmahat^{(m)} - \Sigma||_{\mathsf{op}} \leq \gamma \epsilon ,
\end{align*}

where the last step follows by standard arguments on the concentration of the empirical covariance matrix directly give us the result.

We will now use this to prove both Equation~\eqref{eq:opnormcontrol} and~\eqref{eq:opnormequationsc}.
To show Equation~\eqref{eq:opnormequationsb}, we first note that $\widetilde{R} - \Rhat = \Tgamma{\Sigma}^{-1} - \Sigmahat^{-1}$.
Then, we get$(\Tgamma{\Sigma})^{-1} - \Sigmahat^{-1} = (\Tgamma{\Sigma})^{-1}(\Sigmahat - \Tgamma{\Sigma}) \Sigmahat^{-1}$ and by the Cauchy-Schwarz inequality on the operator norm, we get
\begin{align*}
    (\Tgamma{\Sigma})^{-1} - \Sigmahat^{-1} &\leq ||(\Tgamma{\Sigma})^{-1}||_{\mathsf{op}} ||\Sigmahat^{-1}||_{\mathsf{op}} ||\Sigmahat - \Tgamma{\Sigma}||_{\mathsf{op}} \\
    &\leq \frac{1}{\gamma^2} ||\Sigmahat - \Tgamma{\Sigma}||_{\mathsf{op}} \leq \frac{\epsilon}{\gamma}
\end{align*}

where the second-to-last inequality is a consequence of the definition of the truncation operation in Definition~\ref{def:thresholdingoperator}.
This shows Equation~\eqref{eq:opnormequationsc}.
Similarly, Equation~\eqref{eq:opnormcontrol} follows because we have
\begin{align*}
    ||\Tgamma{\Sigma}^{-1/2} \Sigmahat \Tgamma{\Sigma}^{-1/2} - I||_{\mathsf{op}} \leq ||\Tgamma{\Sigma}||_{\mathsf{op}} \cdot ||\Sigmahat - \Tgamma{\Sigma}||_{\mathsf{op}} = \frac{1}{\gamma} \cdot \gamma \epsilon = \epsilon .
\end{align*}

This completes the proof.
\end{proof}

With the proof of Lemma~\ref{lem:opnormcontrol} complete, we have completed the proof of Theorem~\ref{thm:truncatedestimator}.

\end{proof}

==> proof_sketch.tex <==
%!TEX root = modelselection_alt2022.tex

\section{Proof sketches}\label{sec:proofsketches}

\subsection{Universal model selection}\label{sec:proofsketchuniversal}

\subsection{Data-adaptive model selection}\label{sec:proofsketchdataadaptive}

==> setting.tex <==
%\usepackage[papersize={17cm,24cm},margin=18mm,top=17mm,headsep=5mm]{geometry} 
%\usepackage[papersize={17cm,24cm},margin=13mm,top=17mm,headsep=5mm]{geometry} 
%\usepackage[utf8]{inputenc}
%\usepackage{xltxtra} % extras for XeLaTeX
%\usepackage{unicode-math}
\usepackage{fullpage}
\usepackage{epsf}
\usepackage{fancyhdr}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{psfrag}
\usepackage[T1]{fontenc}
\usepackage{color}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{accents}
\usepackage{listings}
\usepackage{caption}
\usepackage{subcaption}
\usepackage[linesnumbered, ruled, vlined]{algorithm2e}
\usepackage[titletoc,toc,title]{appendix}
\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-6cm}
\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-4cm}
\addtolength{\textheight}{-1.1\headheight}
\addtolength{\textheight}{-\headsep}
\addtolength{\textheight}{-\footskip}
\setlength{\oddsidemargin}{0.5cm}
\setlength{\evensidemargin}{0.5cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
  \settoheight{\widebarargheight}{\ensuremath{#1}}%
  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
    \hspace{0.3\widebarargdepth}%
    \addtolength{\widebarargheight}{0.3ex}%
    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
  {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
        \vskip 0.8ex
        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
        \parindent 1.5em  %% How can we use the global value of this???
        \dimen0=\hsize
        \advance\dimen0 by -3em
        \ifdim \wd\@tempboxa >\dimen0
                \hbox to \hsize{
                        \parindent 0em
                        \hfil 
                        \parbox{\dimen0}{\def\baselinestretch{0.96}\small
                                {\bf #1.} #2
                                %%\unhbox\@tempboxa
                                } 
                        \hfil}
        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
        \fi
        }
\makeatother


\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage{times}
\usepackage{enumerate}
\usepackage{verbatim} % verbatim input
%\usepackage{titling} % customize title
\usepackage[titletoc,toc,title]{appendix}
\usepackage{csquotes} % context sensitive quotes
\usepackage{upquote} % allow correct quotes in verbatim
\usepackage[bottom]{footmisc} % put footnotes down at the bottom margin
%\usepackage[svgnames]{xcolor} % color pictures with SVG names
\usepackage{graphicx} % \includegraphics
%\usepackage[noend]{algpseudocode}
\usepackage[ruled]{algorithm2e}
\usepackage{thmtools}
\usepackage{thm-restate}
%\usepackage{tikz}
%\usetikzlibrary{matrix,shapes,arrows,positioning,chains, calc}
%\usepackage[dvipsnames]{xcolor}
\usepackage[dvipsnames]{xcolor}
%\usepackage{lmodern}
%\usepackage{authblk}
%\usepackage{hyperref}
\usepackage[colorlinks,linkcolor = RawSienna, urlcolor  = violet, citecolor = RoyalBlue, anchorcolor = violet]{hyperref}
\usepackage{cleveref}
%\usepackage[colorlinks,linkcolor = blue, urlcolor  = green, citecolor = Aquamarine, anchorcolor = blue]{hyperref}
%\usepackage{optidef}
%\usepackage{enumitem} % customize lists
%\setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
%\setitemize{itemsep=2pt,topsep=4pt,parsep=0pt,partopsep=0pt}
%\usepackage{covington}  % for numbered linguistic examples

\usepackage[english]{babel} % multilinguality
%\usepackage{polyglossia} % newer alternative to babel
%\setdefaultlanguage{english} % see http://ctan.uib.no/macros/xetex/latex/polyglossia/polyglossia.pdf
%\setmainfont[Mapping=tex-text,Ligatures=TeX,Scale=1.0]{Linux Libertine O} 
%\setmonofont[Mapping=tex-text,Scale=MatchLowercase,LetterSpace=-2.0]{DejaVu Sans Mono}
%\setmathfont{Cambria Math}
%\setmathfont[math-style=upright,vargreek-shape=unicode]{Neo Euler}
%\setmathfont{Linux Libertine O}
\renewcommand{\baselinestretch}{1.04} % stretch distance between baselines
\frenchspacing % reduce space after sentence-final punctuation
\date{}
\setlength{\parindent}{1em}
\clubpenalty = 10000
\widowpenalty = 10000
\hfuzz = 2pt  % No warnings about margin overhangs less than this amount.
%\setlength{\belowcaptionskip}{-1.2em}
%Theorem Repeat solutions


%\usepackage[compact,noindentafter]{titlesec} % customize section headings
%\titlespacing{\section}{0pt}{2.7mm}{1.5mm} % left indent, space before, space after
%\titlespacing{\subsection}{0pt}{2mm}{1pt}
%\titlespacing{\subsubsection}{0pt}{1.2mm}{0.5pt}

%\newcommand\Volume{N} % BeLLS Volume number
%\newcommand\Voleditors{Jan Editor and Ed Janitor}
%\newcommand\Voltitle{The book title}
%\newcommand\VolISBN{N}
%\newcommand\VolDOI{N}

%\usepackage{natbib}
\usepackage[style = alphabetic,citestyle=alphabetic,maxbibnames=99,backend=biber,natbib=true,backref=true]{biblatex}
\addbibresource{ref.bib}
\DefineBibliographyStrings{english}{%
  backrefpage = {Cited on page},% originally "cited on page"
  backrefpages = {Cited on pages},% originally "cited on pages"
}
%\usepackage{fullname}
%\bibliographystyle{plain}
%\bibliographystyle{chicago} % chicago or spbasic or spmpsci or spphys
%\bibliographystyle{alphanat} % chicago  or spbasic or spmpsci or spphys
%\setlength{\bibhang}{-0.5em}
%\setlength{\bibsep}{0mm}
%\let\bibfont=\small
%\setcitestyle{numbers}

% footnote without number
% \newcommand\blfootnote[1]{
%   \begingroup
%   \renewcommand\thefootnote{}\footnote{\hspace{-2.4em} #1}%
%   \addtocounter{footnote}{-1}
%   \endgroup
% }

% customize title
%\renewcommand{\maketitle}
%  {\bgroup\setlength{\parindent}{0pt}
%   \begin{flushleft}
%    \textbf{\LARGE{\ \\ \vspace{20mm}\strut\thetitle\strut}\vspace{2mm}}
%    
%    {\Large\theauthor}
%  \end{flushleft}\egroup\vspace{18mm}
%}

%% customize abstract
%\renewenvironment{abstract}
%  {\noindent\small %\quotation
%  {\noindent{\large\textbf\abstractname. }%\par\nobreak\smallskip
%  \thispagestyle{plain}
%  %\blfootnote{In: \emph{Volume title,} edited by Jan Editor and Ed Janitor. BeLLS Vol. N (2017), DOI N. Open Access under the terms of CC-BY-NC-4.0.}
%  }}
%  {}
%    
%% command in which to embed tabular material in numbered example
%% use: \begin{example}\extab\begin{tabular ...
%\newcommand{\extab}[2][-0.69\baselineskip]{ 
%   \parbox[t]{.9\textwidth}{
%     \setlength{\tabcolsep}{1.3pt} % use small space between columns
%     \vspace{#1}
%     #2
%    }
%}

% command to put ref in parentheses
\newcommand{\refp}[1]{(\ref{#1})}
  
%user defined commands
\newcommand*\Mirr[1]{\textsc{Mirr} (#1)}
\newcommand*\Wd[0]{\textit{W}_2}
\newcommand*\dd[2]{\frac{\partial #1}{\partial #2}}
\newcommand*\x[0]{\textbf{x}}
\newcommand*\stein[1]{\mathcal{A}_{#1}}
\newcommand*\w[0]{\textbf{w}}
\newcommand*\at[2]{\left.#1\right|_{#2}}
\newcommand*\ps[0]{p^*}
\newcommand*\del[0]{\partial}
\newcommand*\R[0]{\mathbb{R}}
\newcommand*\Z[0]{\mathbb{Z}}
\renewcommand*\div[0]{\nabla \cdot}
\newcommand*\ddt[0]{\frac{d}{d t}}
\newcommand*\dds[0]{\frac{d}{d s}}
\newcommand*\ddp[1]{\frac{\delta #1}{\delta p}}
\newcommand*\tr[0]{\text{tr}}
\newcommand*\KL[2]{\mathcal{KL}\left(#1\|#2\right)}
\newcommand*\lin[1]{\langle #1\rangle}
\newcommand*\E[1]{\mathbb{E}\left[#1\right]}
\newcommand*\Ep[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand*\grad[3]{\mathcal{D}_{#1}(#2,#3)}
\newcommand*\slope[1]{\|\mathcal{D}_{#1}\|}
\newcommand*\md[1]{\|\frac{d}{dt}#1\|}
\newcommand*\ap[2]{\tilde{#1}_{#2}}
\newcommand*\F[0]{\mathcal{F}}
\newcommand*\D[0]{\mathcal{D}}
\renewcommand*\H[0]{\mathcal{H}}
\newcommand*\Pspace[0]{\mathscr{P}}
\newcommand*\Uspace[0]{\mathbb{U}}
\renewcommand*\t[1]{\tilde{#1}}
\renewcommand*\d[0]{\text{d}}
\newcommand*\ot[1]{#1^{\perp}}
\newcommand*\proj[0]{\text{Proj}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand*\lrb[1]{\left[#1\right]}
\newcommand*\lrp[1]{\left(#1\right)}
\newcommand*\eu[1]{\left\| #1\right\|}
\renewcommand*\div[0]{\nabla \cdot}
\renewcommand*\H[0]{\mathcal{H}}
\renewcommand*\t[1]{\tilde{#1}}
\renewcommand*\d[0]{\delta}
\newcommand*\xt[0]{\tilde{x}}
\newcommand*\vt[0]{\tilde{v}}
\newcommand*\pt[0]{\tilde{p}}
\newcommand*\qt[0]{\tilde{q}}
\newcommand*\Phit[0]{\tilde{\Phi}}
%NewSymbols
\def\ci{\perp\!\!\!\perp}
\def\half{\frac{1}{2}}
\def\lv{\lVert}
\def\rv{\rVert}
\def\ke{\mathcal{K}}
\def\kc{\hat{\mathcal{K}}_m}
\DeclareMathOperator{\Tr}{tr}


\newcommand*\diff{\mathop{}\!\mathrm{d}}

\newcommand{\note}[1]{\textbf{{\color{red}#1}}}
\newcommand{\rem}[1]{{\emph{#1}}}


\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\newenvironment{Proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

\newcommand\psued[1]{R^s_{#1}}

\newcommand\regret[1]{R^c_{#1}}

\newcommand\ind[2]{\mathbb{I}_{#1,#2}}
\newcommand\indi[0]{\mathbb{I}}

\newcommand\algname{\mathsf{OSOM}}
\newcommand\UCB{\mathsf{UCB}}
\newcommand\OFUL{\mathsf{OFUL}}
\newcommand\corral{\mathsf{CORRAL}}
\newcommand\moss{\mathsf{MOSS}}
\newcommand\linucb{\mathsf{LinUCB}}
\newcommand\expalg{\mathsf{EXP}4}
\newcommand\expsim{\mathsf{EXP}3}
\newcommand\sao{\mathsf{SAO}}

\newcommand\tstar{\tau_*}
\usepackage[shortlabels]{enumitem}
\newcommand\unitball{\mathbb{B}_2^d(1)}

\newcommand\mustar[1]{\mu_{#1}}
\newcommand\nustar[1]{\nu_{#1}}
\newcommand\thetastar{\theta^{*}}

\newcommand\tinrange[2]{t \in \{#1,\ldots, #2\}}
\newcommand\sinrange[2]{s \in \{#1,\ldots, #2\}}
\newcommand\iinrange[2]{i \in \{#1,\ldots, #2\}}
\newcommand\Xt{X_{t}}
\newcommand\Xs{X_{s}}
\newcommand\Xit[2]{X_{#1,#2}}
\newcommand\alpt[2]{\alpha_{#1,#2}}
\newcommand\betat[2]{\beta_{#1,#2}}

\newcommand\muit[2]{\tilde{\mu}_{#1,#2}}

\newcommand\gis{g_{i,s}}
\newcommand\git{g_{i,t}}

\newcommand\ccomplex{\mathcal{C}_t^c}
\newcommand\csimple{\mathcal{C}_t^s(i)}

\newcommand\mconstraint{V_t}

\newcommand\Ostar{\Omega^*}
\newcommand\Otilde{\tilde{\Omega}_t}
\newcommand\Ohat{\hat{\Omega}_t}

\newcommand\Tstar{\theta^*}
\newcommand\Ttilde{\tilde{\theta}_t}
\newcommand\That{\hat{\theta}_t}


\newcommand\Xboldt{\mathbf{X}_{1:t}}
\newcommand\Aboldt{\boldsymbol{\alpha}_{K+1:t}}
\newcommand\Gboldt{\mathbf{G}_{K+1:t}}

\newcommand\Xboldtn{\mathbf{X}}
\newcommand\Aboldtn{\boldsymbol{\alpha}}
\newcommand\Gboldtn{\mathbf{G}}
\newcommand\etabold{\boldsymbol{\eta}}
\newcommand\mubold{\boldsymbol{\mu}}
\newcommand\mutbold{\boldsymbol{\tilde{\mu}}}

\newcommand\averagerew{\bar{g}_{i,t}}

\newcommand\Otildes{\tilde{\Omega}_s}
\newcommand\Ohats{\hat{\Omega}_s}

\newcommand\tmin{\tau_{\min}(\delta',T)}
\newcommand\updela{\Upsilon_{\delta'}(t,T)}
\newcommand\mone{\mathcal{M}_{\delta'}(t)}
\newcommand\mtwo{\mathcal{M}_2}
\newcommand\kenv{\mathcal{K}_{\delta'}(t,T)}
\newcommand\kenvs{\mathcal{K}_{\delta'}(s-1,T)}
\newcommand\kenvt{\mathcal{K}_{\delta'}(t,T)}
\newcommand\wenv{\alpha_{\delta'}(t,T)}
\newcommand\wenvone{\alpha_{\delta'}(t,T)}
\newcommand\wenvtau{\alpha_{\delta'}(\tstar-1,T)}
\newcommand\wenvn{\alpha_{\delta'}(T,T)}
\newcommand\wenvnre{\alpha_{\delta'}(T,T)}
\newcommand\bfm[1]{\mathbf{#1}}
\newcommand\loweig{\gamma}
\newcommand\higheig{\rho_{\max}}

\newcommand\Oh{\mathcal{O}}

\usepackage{mathtools}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
%\renewcommand{\tilde}{\widetilde}




%%%%NEW MACROS FOR NEW IDEAS!
\newcommand\Rhat{\widehat{R}}
\newcommand\Dhat{\widehat{D}}
\newcommand\Sigmahat{\widehat{\Sigma}}
\newcommand\Sigmabar{\overline{\Sigma}}
\newcommand\Omegahat{\widehat{\Omega}}
\newcommand\Sigmagamma{[\Sigma]_{\gamma}}
\newcommand*\Tgamma[1]{T_{\gamma}\left(#1\right)}
\newcommand\Uhat{\widehat{U}}
\newcommand\Lambdahat{\widehat{\Lambda}}
\newcommand\lambdahat{\widehat{\lambda}}
\newcommand\Sgaphat{\widehat{\mathcal{E}}}
\newcommand\Sgaptilde{\widetilde{\mathcal{E}}}
\newcommand\Sgap{\mathcal{E}}
\newcommand\Sgapbar{\overline{\mathcal{E}}}
\newcommand\tildex{\widetilde{x}}
\newcommand\Ecal{\mathcal{E}}
\newcommand\tauswitch{\tau_{\mathsf{switch}}}
\newcommand\mutilde{\widetilde{\mu}}

\newcommand\T{\mathcal{T}}
\newcommand\W{\mathcal{W}}

\newcommand\vm[1]{\textcolor{blue}{VM -- #1}}
\newcommand\ak[1]{\textcolor{red}{AK -- #1}}
